TimeArena: Shaping Efficient Multitasking Language Agents in a Time-Aware Simulation

Despite remarkable advancements in emulating human-like behavior through Large Language Models (LLMs), current textual simulations do not adequately address the notion of time. To this end, we introduce TimeArena, a novel textual simulated environment that incorporates complex temporal dynamics and constraints that better reflect real-life planning scenarios. In TimeArena, agents are asked to complete multiple tasks as soon as possible, allowing for parallel processing to save time. We implement the dependency between actions, the time duration for each action, and the occupancy of the agent and the objects in the environment. TimeArena grounds to 30 real-world tasks in cooking, household activities, and laboratory work. We conduct extensive experiments with various state-of-the-art LLMs using TimeArena. Our findings reveal that even the most powerful models, e.g., GPT-4, still lag behind humans in effective multitasking, underscoring the need for enhanced temporal awareness in the development of language agents.

==> archived/010intro_2_7_backup.tex <==

Large language models (LLMs)~\cite{openai2022chatgpt,openai2023gpt4,geminiteam2023gemini,Hugo2023LLaMa,Hugo2023LLaMa2} have enabled the development of language agents (\textit{a.k.a.} LLM-based agents), which aim to simulate human behaviors in real-world scenarios through their reasoning and planning capabilites~\cite{wu2023smartplay,liu2023agentbench,gong2023mindagent,akata2023playing}.
However, planning in the real world involves temporal and resource constraints~\cite{russell2010artificial}, which are rarely implemented in most textual simulations for LLMs and language agents~\cite{wang-etal-2022-scienceworld,park2023generative}.





\definecolor{mygray}{RGB}{233,233,233}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/front.pdf}
    \caption{An example illustrating multitasking with temporal constraints in \method.
    The completion of tasks requires actions in a predetermined dependency and order. 
    \underline{Underlined actions} do not occupy the agent, allowing other actions to be processed by the agent simultaneously. 
    The \colorbox{mygray}{Wait} action skips the current time step, meaning the agent is idle.
    }
    \label{fig:front}
\end{figure}

The integration of time in simulated environments challenges agents to navigate and align with human-like efficient multitasking skills.
Such a simulation requires the agent to consider the following three factors:
\begin{inparaenum}[1)]
    \item \textbf{Time Duration and Dependency:} Actions will have durations upon dependencies, requiring agents to strategize and prioritize based on time constraints and task completion progress.
    \item \textbf{Agent Occupancy:} Agents will be occupied by certain actions thus they might be unable to perform other actions at the same time.
    \item \textbf{Object Occupancy:} 
    Some objects might be occupied for some time, and agents must use available objects in the environment for the tasks. 
\end{inparaenum}
These factors are common in real-life but are seldom addressed by current textual simulations.


To help illustrate,
Figure~\ref{fig:front} shows an example of completing the task of ``make tea'' (Task 1) and ``wash clothes'' (Task 2).
The actions of each task might depend on previous actions (\eg, agents must \coloredtexttt{boil water} before \coloredtexttt{make tea}.), and each action takes a specific duration in time (\eg, \coloredtexttt{wash cup} takes 5 minutes).
In particular, some actions let agents be idle, allowing agents to carry out other actions.
For example, \coloredtexttt{wash clothes in washing machine} allows agents to perform other actions at the same time.
Moreover, actions temporarily occupy objects, making them unavailable for other actions and hindering parallel processing. 
For example, \coloredtexttt{boil water} occupies the \coloredtexttt{pot}, delaying other actions like \coloredtexttt{cook soup} until it is available.
When no action is currently available for the agent, the only option is to wait. 
For example, in Solution 2, the agent must wait for the completion of \coloredtexttt{wash clothes in washing machine}, before \coloredtexttt{hang clothes}.


In this work, we introduce \method, a textual simulated environment featuring 30 real-world involving cooking, household activities, and laboratory work.
\method is the first textual simulation to evaluate language agents on multitasking efficiency.
Specifically, we incorporate the time duration of each action and set two types of actions based on agent occupancy.
One type occupies agents (\eg, \coloredtexttt{wash cup}) and another lets agents be idle (\eg, \coloredtexttt{boil water}). 
Additionally, we simulate resource competition by implementing object occupancy, i.e., an object used for one task cannot be simultaneously used for another, which is common in parallel processing. 
Therefore, agents must focus on parallel processing, taking into account the occupancy of agents and objects, to minimize time consumption.
We design four metrics in \method to evaluate the average progress, completion speed, task completion rate and average completion time.
These metrics help to assess and analyze the efficient multitasking capabilities of language agents. 
Our comprehensive evaluation of 7 LLMs on \method shows that current language agents struggle in efficient multitasking.
Even the most powerful LLM, GPT-4, still faces challenges in parallel processing.



In summary, our contributions are as follows:
\begin{inparaenum}[\it 1)]
    \item To the best of our knowledge, we are the first to explore the notion of time of language agents in a textual environment, which is important for more realistic simulation.
    \item We create \method, a novel text-based simulated environment consisting of 30 tasks, where LLMs can complete multiple tasks in parallel.
    \item Using \method, we conduct rich experiments to evaluate the efficient multitasking capabilities of language agents. Our results demonstrate that efficient multitasking in \method poses a significant challenge for current LLMs and language agents.
\end{inparaenum}




==> archived/015introduction.tex <==

Large language models (LLMs)~\cite{openai2022chatgpt,openai2023gpt4,geminiteam2023gemini,Hugo2023LLaMa,Hugo2023LLaMa2} have recently sparked interest in LLM-based agents (language agents), which aim to simulate human behaviors and interact with the real-world scenarios through their reasoning and planning capabilites~\cite{wu2023smartplay,liu2023agentbench,gong2023mindagent,akata2023playing}.
However, there is a missing piece in the simulated environments and the evaluation of these agents~\cite{wang-etal-2022-scienceworld,park2023generative} that prevents them from stepping into the real world: the notion of \textit{time}, which is crucial in the spacetime in which we live.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/front.pdf}
    \caption{An example illustrates multitasking within time constraints.
    Tasks necessitate actions in a predetermined dependency order. 
    \underline{Underlined actions} do not require continuous performing, allowing other actions to be processed simultaneously. 
    Agents striving for the quickest task completion find parallel processing more efficient than serial processing.}
    \label{fig:front}
\end{figure}

Integrating ``time'' into simulated environments for agents introduces new dimensions and challenges to task management.
\sout{Tasks will have durations on top of dependencies} \cjj{tasks or actions? be clear and consistent with sec 3.}, requiring agents to strategize and prioritize based on time constraints and sequential task completion.
Agents, \sout{occupied with tasks for set periods} \cjj{need to be consistent with sec 3.}, must balance their time budget, unable to perform multiple activities simultaneously.
This mimics human multitasking limitations.
Additionally, the requirement for specific objects, occupied for certain durations, adds complexity, as agents must manage resource availability alongside task scheduling.
Thus, this integration of time in simulated environments challenges language agents to navigate and align with human-like multitasking and decision-making processes.


To illustrate how multitasking with time constraints works, Figure~\ref{fig:front} shows an example of completing the task of making tea (task 1) and washing clothes (task 2).
The actions of each task might depend on previous actions (\eg, agents must \coloredtexttt{boil water} before \coloredtexttt{bake tea}.), and each action takes a specific duration in time (\eg, \coloredtexttt{wash cup} takes 5 minutes).
In particular, some actions do not need to be done continuously, which means that \sout{these actions do not let agent be occupied} \cjj{what do you mean by not let agent be occupied? lack clear, concise explanation of occupancy.}).
For example, \coloredtexttt{boil water} and \coloredtexttt{wash clothes in washing machine} \sout{can} \cjj{use less ``can xxx'', very Chinglish.} allow agents \sout{do} \cjj{stay consistent with ``perform actions''} other actions at the same time.
Moreover, actions can temporarily occupy objects, \sout{affecting the ability to perform multiple tasks at once} \cjj{unclear. example should be straightforward, e.g., ``making them unavailable for other actions and thus hindering multi-tasking''}. 
For example, \coloredtexttt{boil water} occupies the \coloredtexttt{pot}, delaying other actions like \coloredtexttt{cook soup} until it is available.















In this paper, we aim to evaluate the notion of time in LLM-based agents by embedding \textit{time} into a simulated environment.
However, it is nontrivial to create such a \sout{simulated} environment due to the following challenges:
1) the simulation must handle complex dependencies between actions to avoid the simultaneous execution of interdependent actions;
2) \sout{additionally,} the simulation should realistically reflect the \sout{agents' states, determining their capability for concurrent actions} \cjj{what is ``agents states''? use straightforward words, leave formal definition later in sec 3.};
3) \sout{the state of objects within the environment is crucial when introducing the notion of time, since actions directed at specific objects can temporarily render them occupied.} \cjj{compress this sentence. too verbose. make it simple and clear.} 
Once an \sout{action's duration is factored in} \cjj{weird phrase}, the object remains occupied for that period.
The environment must manage resource allocation effectively, releasing or occupying resources as actions dictate and restricting agents from accessing occupied objects.
\cjj{I think this sentence could be improved. maybe refer to sec 3.3 feedback section.}






To address the above challenges, we introduce \method, a text-based \sout{virtual} \cjj{simulated} environment featuring 30 real-world tasks in cooking, \sout{household} \cjj{use householding}, and laboratory scenarios.
\method is the first \cjj{textual simulation (it's important to pick your lane, you don't want to mess with real games.)} to integrate the notion of time to evaluate the capabilities of LLM-based agents on multitasking ability in \sout{real-world scenarios} \cjj{I'd be careful with this term.}.
Specifically, we go beyond simply considering the dependency of actions by incorporating their duration, a critical aspect in modeling time.
The duration of actions can either limit \sout{continuous involvement} \cjj{what does this mean?} of \sout{LLM-based} \cjj{mention once is enough.} agents (e.g., \coloredtexttt{wash cup}) or enable them to handle multiple tasks simultaneously (e.g., \coloredtexttt{boil water} and \coloredtexttt{sweep floor} concurrently).
Additionally, we simulate resource competition common in parallel task execution by considering object occupancy. 
LLM-based agents must schedule multiple tasks with these resource constraints, ensuring that an object in use for one task cannot be simultaneously used for another.
To interact with \method, agents receive environmental feedback and \sout{a reward score} \cjj{be consistent with sec 3.} for each action which \sout{can} helps them in \sout{future task decomposition and action planning} \cjj{why is it helpful for these? explain.}.
\sout{Therefore, LLM-based agents must focus on parallel processing, taking into account the duration of actions and object occupancy, to minimize time consumption and maximize the total reward score when completing multiple tasks.}
\cjj{Compress this sentence.}


We design four evaluation metrics, \ie, average score, completion velocity, task completion rate and average completion time.
These metrics help assess and analyze the \sout{multitasking scheduling} \cjj{be consistent} capabilities of LLM-based agents from various perspectives. 
We conduct extensive experiments on multiple LLMs to explore their ability to understand dependencies and parallel processing between actions. 
\sout{The results demonstrate that multitasking scheduling in \method continues to pose a significant challenge for current LLM-based agents.} \cjj{move to contribution, maybe} 
In summary, our contributions are as follows:





\begin{itemize}
    \item To the best of our knowledge, we are the first to explore the notion of time of LLM-based agents in multitasking scheduling. \cjj{again, pick your lane.}
    \item We create \method, a text-based simulated environment consisting of 30 \sout{real-world} tasks, to enable LLMs to \sout{parallel schedule multiple tasks} \cjj{be consistent} in three different scenarios.
    \item Using \method, we conduct extensive experiments to evaluate and analyze the \sout{multitasking scheduling} capabilities of LLM-based agents from various perspectives. \cjj{move here}
\end{itemize}









==> archived/030method_2_7_backup.tex <==


We create \method, a textual simulated environment to evaluate the efficient multitasking capabilities of language agents.
To help illustrate, we first show an overview and an example run of how an agent interacts with the \method environment ($\mathsection$~\ref{sec3:overview}), and then describe the design of the simulation environment in more detail ($\mathsection$~\ref{sec3:components}-\ref{sec3:feedback}).



\subsection{Overview of \method}
\label{sec3:overview}









\method challenges agents to complete multiple tasks strategically in the shortest possible time. 
This simulation emphasizes the importance of understanding, performing, and optimizing actions within a constrained timeframe, mirroring practical scenarios involving time management.

Central to \method are \textbf{Tasks}, \textbf{Objects}, and \textbf{Actions}. \textbf{Tasks} define the objectives for the agents, \textbf{Objects} represent elements in the environment that agents will encounter and interact with, and \textbf{Actions} are the means to accomplish these tasks. 
Real-time feedback and scoring mechanisms are integral to the environment, assessing agent performance and adding to the simulation's complexity and realism. 
Unique features like the duration and occupancy of actions and strategic resource utilization distinguish \method from other environments.

\paragraph{An Example Run}
As in Figure~\ref{fig:TimeArena}, consider an agent tasked with ``make tea'' (Task 1), ``wash clothes'' (Task 2) and ``wash bed sheet'' (Task 3).
The agent starts by decomposing the task into actions like \coloredtexttt{boil water}.
In \method, all actions have a duration (\eg, \coloredtexttt{Boil water} needs 8 minutes.) and dependencies (\eg, At T=4min, \coloredtexttt{make tea} violates the dependency because \coloredtexttt{wash teapot} and \coloredtexttt{boil water} are not completed yet.).
The agent then interacts with objects (e.g., \coloredtexttt{wash clothes in washing machine}), which become \textbf{occupied} during the process. 
The agent can engage in non-occupied
actions simultaneously (e.g., \coloredtexttt{wash teapot}) while others (e.g., \coloredtexttt{boil water}) are in progress.
Environmental feedback guides the agent, indicating the legitimacy of actions and the completion of tasks. 
For example, if the \coloredtexttt{washing machine} is occupied, the agent adjusts its strategy. 
The agent's goal is to complete all tasks efficiently, with performance evaluated based on progress and completion time.

This dynamic interaction in \method fosters an environment where strategic planning, resource management, and adaptability are key to an agent's success.

 


\subsection{Components of \method}
\label{sec3:components}

\paragraph{Tasks}
In \method, We design tasks within three distinct \textit{scenarios} or simulated settings, namely, \textit{household activities}, \textit{cooking}, and \textit{laboratory work}.
Each scenario represents a specific context or environment where multitasking is an integral part of the activities involved.\footnote{Details of tasks are in Appendix~\ref{app:task}.}
For example, one can do a \coloredtexttt{sweep floor} while doing \coloredtexttt{boil water}, and do a \coloredtexttt{wash dishes} while doing \coloredtexttt{cook soup}.
Each scenario contains 10 tasks,
and some actions and objects are shared across multiple tasks of a scenario.
Each task requires multiple actions to be executed, which manipulates the objects in the environment for task completion.
In the beginning, \method gives a list of tasks to the agent, with a comprehensive task instruction consisting of a \textit{task description}, an \textit{action space}, and an \textit{object set}:
\begin{itemize}[noitemsep]
    \item \textbf{Task Description}: Introduces task objectives (\eg, ``Task 1: Make a dish of beef fried rice, which consists of cooked rice and fried beef.'');
    \item \textbf{Action Space}: Lists the valid actions for the tasks (\eg, \coloredtexttt{chop}, \coloredtexttt{wash});
    \item \textbf{Object Set}: Lists the available objects in the environment for the tasks (\eg, \coloredtexttt{pot}, \coloredtexttt{beaker}).
\end{itemize}
At every timestep $t$, the agent needs to generate valid actions on the objects and receive feedback from the environment.

\paragraph{Objects}
Objects are integral to completing tasks and situating within the environment.
In \method, there are 71 different objects for all the tasks.
Every task involves a list of objects, which might overlap with other tasks of the same scenario.
To mimic the resource limitation in real-world parallel processing, we introduce:
\begin{itemize}
    \item \textbf{Object Occupancy}: the state of the object involved in an action is set to be \textit{occupied}, \eg, \coloredtexttt{wash cup} will cause the object \coloredtexttt{cup} to be occupied.
    This object cannot be processed until the involved action is completed (after some time).
    Then, this object is reset as non-occupied and waits for another action.
\end{itemize}



\paragraph{Actions}

We design a total of 45 actions for all 30 tasks.
Each action consists of a detailed description (\eg, \coloredtexttt{chop OBJ}, \coloredtexttt{chop the whole item into sliced pieces.}), showing a change of states the action will cause to an object.\footnote{All the actions are listed in Apendix~\ref{app:action}.}
Different from existing text-based simulations~\cite{wang-etal-2022-scienceworld,gong2023mindagent,shridhar2020alfworld}, in our case, an action has a duration of time and may occupy the agent from performing other actions, to the passage of time.
In detail:
\begin{itemize}[noitemsep]
    \item \textbf{Action Dependency}: An action within the same task might depend on completing other actions within the same task. 
    As depicted in Figure~\ref{fig:TimeArena}, \coloredtexttt{make tea} is dependent on \coloredtexttt{wash teapot}.
    \item \textbf{Duration of Time}:
    Each action holds a timeframe in the timeline, ranging from 1 to 10 minutes.
    In practice, agents only have an educated guess of the time duration of each action until actually interacting with \method.  
    \item \textbf{Agent Occupancy}:  
    One key to parallel processing is agent occupancy, which prevents agents from performing other tasks.
    Therefore, we consider two types of actions based on agent occupancy:
    1) Type 1 action occupies the agent til completion (\eg, \coloredtexttt{wash teapot}); and 2) Type 2 action lets agents be idle, allowing to perform other actions (\eg, \coloredtexttt{boil water}).
\end{itemize}


\subsection{Agent Interaction and Environmental Feedback}
\label{sec3:feedback}
\paragraph{Environmental Feedback}
The feedback from a textual environment is important to simulate and implement the constraints in \method using only textual messages.
We define feedback as the response from the environment following an action by an agent.
A feedback message could be of multiple types, including:
\begin{itemize}[noitemsep]
    \item \textbf{Invalid Action}:
    An action attempt that does not match the required format, \eg, \textit{``\coloredtexttt{clean teapot} is invalid''}.
    \item \textbf{Action on Non-existing Object}:
    An action attempt that visits objects that are not in the object set, \eg, \textit{``\coloredtexttt{pan} is non-existent''}.
    \item \textbf{Wrong Action Input}:
    An action attempt that the prerequisite action has not completed (\eg, \textit{``Cannot perform action \coloredtexttt{add to} on object \coloredtexttt{shrimp}. Because \coloredtexttt{shrimp} is \coloredtexttt{raw}''.}) or has been completed (\eg, \textit{``\coloredtexttt{wash beaker} has been completed''}).
    \item \textbf{Action on Mismatched Object}:
    An action attempt that does not match the object, \eg, \textit{``You cannot perfrom \coloredtexttt{read} on \coloredtexttt{potato}.''}
    \item \textbf{Action on Occupied Object}:
    An action attempt on occupied objects, \eg, \textit{``Object \coloredtexttt{pot} is being occupied by another action''.}
\end{itemize}
Correspondingly, valid actions will trigger environmental feedback of the following types:
\begin{itemize}[noitemsep]
    \item \textbf{Action Start}:
    Avoiding previous errors,
    valid actions will receive a feedback message containing the specific performing time, marking the start of the action, \eg, \textit{You are doing \coloredtexttt{wash cup}, it will take 9 minutes}.
    \item \textbf{Action Completion}:
    When an action is completed, the environment will send a message, \eg, \coloredtexttt{cup is clean}, and reset the occupying state of the object (\coloredtexttt{cup}).
\end{itemize}


\paragraph{Progress Score}
The progress score, denoted as a percentage, reflects the agent's completion rate of required actions within the environment, where the total duration for all actions is considered as 100\%. 
Each action's contribution to the progress score is proportionate to its duration. 
Specifically, if an action's duration is \(t_i\) minutes, its contribution to the progress score is calculated as \(s_i = \left(\frac{t_i}{\sum_{j=1}^{n} t_j}\right) \times 100\%\), with \(n\) representing the total number of actions. 
For instance, an action lasting 5 minutes in a total action duration of 20 minutes contributes 25\% to the progress score.



==> archived/035method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/main.pdf}
    \caption{An overview of \method. Given a set of tasks, agents perform actions and \method returns feedback. In \method, all actions have duration and dependencies (\eg, At T=6min, \coloredtexttt{make tea} violates the dependency because \coloredtexttt{wash teapot} is not completed yet.). Actions decide the occupancy of agent. Some actions (underlined) will not cause agent to be occupied (\eg, when doing \coloredtexttt{boil water}, agents can \coloredtexttt{sweep floor} and \coloredtexttt{boil water} complete automatically at T=8min.). Other actions need agents doing continuously (\eg, during \coloredtexttt{sweep floor}, agent cannot perform other action.). Furthermore, actions wil occupy objects. For exapmle, \coloredtexttt{boil water} will occupy \coloredtexttt{pot} until the action is finished.
    \todo{to be updated}
    }
    \label{fig:TimeArena}
\end{figure*}

In this paper, as shown in Figure~\ref{fig:TimeArena}, we create \method, a text-based simulated environment to evaluate the multitasking and parallel processing capabilities of language agents.
To help illustrate, we first show an overview and an example run of how an agent interacts with the \method environment ($\mathsection$~\ref{sec3:overview}), and then introduce the important concepts and designs in the environment in detail ($\mathsection$~\ref{sec3:components}-\ref{sec3:feedback}).


\todo{The examples here, including all with \coloredtexttt{xxx}, should be consistent with Fig 1 or Fig 2.}

\subsection{Overview of \method}
\label{sec3:overview}










\method, designed as a text-based game, challenges agents to complete tasks efficiently and strategically in the shortest possible time. This simulation environment emphasizes the importance of understanding, executing, and optimizing actions within a constrained timeframe, mirroring practical scenarios of time management.

Central to \method are \textbf{Tasks}, \textbf{Objects}, and \textbf{Actions}. Tasks define the objectives for the agents, Objects represent elements in the environment to interact with, and Actions are the means to accomplish these tasks. Real-time feedback and scoring mechanisms are integral to the environment, assessing agent performance and adding to the simulation's complexity and realism. Unique features like the duration and occupancy of actions, and strategic resource utilization, distinguish \method from other environments.

\paragraph{An Example Run}
Consider an agent tasked with making a dish of beef fried rice. The agent starts by decomposing the task into actions like \coloredtexttt{chop beef} and \coloredtexttt{cook rice}, estimating the duration for each. The agent then interacts with objects (e.g., \coloredtexttt{washing plate}) which become \textbf{Occupied} during the process. The agent can engage in non-occupying actions simultaneously (e.g., \coloredtexttt{brewing tea}) while others are in progress.

Environmental feedback guides the agent, indicating the legitimacy of actions and the completion of tasks. For example, if the stove is occupied, the agent adjusts its strategy. The agent's goal is to complete all tasks efficiently, with performance evaluated based on progress and completion time.

This dynamic interaction in \method fosters an environment where strategic planning, resource management, and adaptability are key to an agent's success.

\subsection{Components of \method}
\label{sec3:components}

\paragraph{Tasks} 
In \method, we design three scenarios, \ie, \textit{householding}, \textit{cooking}, and \textit{laboratory}, which are common in life for multi-tasking.
For example, \coloredtexttt{sweep floor} while doing \coloredtexttt{boil water}, and \coloredtexttt{wash dishes} while doing \coloredtexttt{cook soup}.
Each scenario contains several tasks (\eg, 10), and actions and objects are shared across multiple tasks of a scenario.
Each task requires a chain of multiple actions to be executed, which manipulates the objects in the environment for task completion.
In the beginning, \method gives a list of tasks to the agent, with a comprehensive task instruction consisting of a \textit{task description}, an \textit{action space} $\mathcal{A}$, and an \textit{object set} $\mathcal{O}$:
\begin{itemize}[noitemsep]
    \item \textbf{Task Description}: Introduces task objectives (\eg, ``Task 1: Make a dish of beef fried rice, which consists of cooked rice and fried beef.'');
    \item \textbf{Action Space}: List the valid actions for the tasks (\eg, ``\todo{fill it}'');
    \item \textbf{Object Set}: List the available objects in the environment for the tasks (\eg, ``\todo{fill it}'').
\end{itemize}
At every timestep $t$, the agent needs to perform valid actions on the objects, and receives feedback from the environment.



\paragraph{Objects}
Objects are integral to completing tasks, situating within the environment.
In \method, there are 71 different objects for all the tasks.
Every task has an object set, which might overlap with other tasks of the same scenario.
To mimic the resource limitation in real world parallel processing, we introduce \textbf{Object Occupancy}: the state of the object involved in an action is set to be \textit{occupied}, \eg, \coloredtexttt{wash cup} will cause the object \coloredtexttt{cup} to be occupied.
This object cannot be processed until the involving action is completed (after some time).
Then, this object is reset as non-occupied and waits for another action.




\paragraph{Actions}

We design a total of 44 actions for all 30 tasks.
Each action consists of a detailed description (\eg, \coloredtexttt{chop OBJ}, \coloredtexttt{chop the whole item into sliced pieces.}), showing a change of states the action will cause to an object. 
Different from existing text-based simulations~\cite{wang-etal-2022-scienceworld,gong2023mindagent,shridhar2020alfworld}, in our case, an action has a duration of time and may occupy the agent from performing other actions, to the passage of time.
In detail:
\begin{itemize}[noitemsep]
    \item \textbf{Action Dependency}: An action within the same task might be dependent on the completion of other actions within the same task. 
    As depicted in Figure~\ref{fig:front}, \coloredtexttt{make tea} is dependent on \coloredtexttt{wash teapot}.
    \item \textbf{Duration of Time}:
    Each action holds a timeframe in the timeline, ranging from 1 to 10 minutes.
    In practice, agents only have an educated guess of the time duration of each action until actually interacting with \method.  
    \item \textbf{Action Occupancy}  
    One key to parallel processing is action occupancy that prevents agents from doing other stuff.
    Therefore, we consider two types of actions based on action occupancy:
    1) Type 1 action occupies the agent til completion (\eg, \coloredtexttt{wash teapot}); and 2) Type 2 action allows agents to do other things (\eg, \coloredtexttt{boil water}).
\end{itemize}


\subsection{Agent Interaction and Environmental Feedback}
\label{sec3:feedback}
\paragraph{Environmental Feedback}
The feedback from a textual environment is important to simulate and implement the constraints in \method using only textual message.
We define feedback as the response from the environment following an action by an agent.
A feedback message could be of multiple types, including:
\begin{itemize}[noitemsep]
    \item \textbf{Invalid Action}:
    An action attempt that does not match the required format.
    \item \textbf{Acting on Non-existing Object}:
    An action attempt that visits objects that are not in the object set.
    \item \textbf{Wrong Action Input}:
    An action attempt that has not completed the prerequisite actions, 
    \eg, \textit{``Cannot perform action \coloredtexttt{add to} on object \coloredtexttt{shrimp}. Because \coloredtexttt{shrimp} is \coloredtexttt{raw}''.}
    \item \textbf{Action on Occupied Object}:
    An action attempt on occupied objects, \eg, \textit{``Object \coloredtexttt{pot} is being occupied by another action''.}.
\end{itemize}
Correspondingly, valid actions will trigger environmental feedback of the following types:
\begin{itemize}[noitemsep]
    \item \textbf{Action Start}:
    Avoiding previous errors,
    valid actions will receive a feedback message containing the specific performing time, marking the start of the action, \eg, \textit{You are doing \coloredtexttt{wash cup}, it will take 9 minutes.}.
    \item \textbf{Action Completion}:
    When an action is completed, the environment will send a message, \eg, \coloredtexttt{cup is clean}, and reset the occupying state of the object (\coloredtexttt{cup}).
\end{itemize}


\paragraph{Progress Score}
The environment also returns the progress score (\%) so far to motivate the agent.
Take the amount of time to complete all actions as 100\%, 
each successfully performed action contributes to the progress score based on its time duration.
Formally, an action takes up $t_i$ minutes, so the completion of it contributes to a progress score $s_i = \frac{t_i}{\sum_{j=1}^{n} t_j} * 100\%$,
where $n$ is the number of all actions in the required tasks.


==> archived/035method_backup.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/main.pdf}
    \caption{An overview of \method. Given a set of tasks, agents perform actions and \method returns feedback. In \method, all actions have duration and dependencies (\eg, At T=6min, \coloredtexttt{make tea} violates the dependency because \coloredtexttt{wash teapot} is not completed yet.). Actions decide the occupancy of agent. Some actions (underlined) will not cause agent to be occupied (\eg, when doing \coloredtexttt{boil water}, agents can \coloredtexttt{sweep floor} and \coloredtexttt{boil water} complete automatically at T=8min.). Other actions need agents doing continuously (\eg, during \coloredtexttt{sweep floor}, agent cannot perform other action.). Furthermore, actions wil occupy objects. For exapmle, \coloredtexttt{boil water} will occupy \coloredtexttt{pot} until the action is finished.
    \todo{to be updated}
    }
    \label{fig:TimeArena}
\end{figure*}

In real scenarios, humans can engage in multitasking to enhance time management and resource utilization. 
For instance, they can simultaneously perform tasks such as \coloredtexttt{chop potato} and \coloredtexttt{boil water}.
The skill of parallel processing plays a key role in boosting efficiency in daily activities.
In this paper, as shown in Figure~\ref{fig:TimeArena}, we create \method, a text-based simulated environment to evaluate the multitasking and parallel processing capabilities of language agents.
In this section, we first give the definition of the task in our simulation ($\mathsection$~\ref{sec:definition}), and then introduce the design of \method ($\mathsection$~\ref{sec:enviroment}). 


\subsection{Task Definition}\label{sec:definition}
We design \method as a text-based simulation, and agents only need to interact with \method using language.
The primary target of language agents in \method is to efficiently schedule actions to complete multiple tasks in the shortest possible time.
At the beginning of the simulation, \method will give a task set that contains multiple tasks.
For each task, \method provides comprehensive instruction for agents, consisting of a task description, an action space $\mathcal{A}$, and an available object set $\mathcal{O}$.
The task description introduces the goal of the task (\eg, ``Task 1: Make a dish of beef fried rice, which consists of cooked rice and fried beef.'').
The action space and object set each list the valid actions and available objects for the task.
At every time $t$, the language agents need to perform valid actions on the objects, and the environment will return score $\mathcal{S}$ and feedback $\mathcal{F}$.
The interaction ends as the time $t$ reaches the maximum number or the score $\mathcal{S}$ accumulate to 100.





\subsection{Environment Design}\label{sec:enviroment}

\paragraph{Scenarios} 
In \method, we design three scenarios, \ie, household, cooking, and laboratory, which are common in life and contain the tasks of parallel processing.
For example, \coloredtexttt{sweep floor} while \coloredtexttt{boil water}, and \coloredtexttt{wash dishes} while \coloredtexttt{cook soup}.
Each scenario includes 10 tasks, with tasks in the same scenario often sharing actions and objects and a task set typically contains multiple tasks in the same scenario.





\paragraph{Actions $\mathcal{A}$}
We design a total of 44 actions for the 30 tasks in three scenarios.
Each action consists of a name with its usage and detailed description (\eg, \coloredtexttt{chop}, \coloredtexttt{chop OBJ}, \coloredtexttt{chop the whole item into sliced pieces.}). 
The usage illustrates how to properly perform actions in \method, and the description shows the changes of states the action will cause to the object.

Different from existing environments~\cite{wang-etal-2022-scienceworld,gong2023mindagent,shridhar2020alfworld}, we further consider durations and occupancy of actions.
\begin{itemize}
    \item \textbf{Duration}
    All the actions have durations in real world.
    To simulate the passage of time during action, we set a duration ranging from 1 to 10 minutes for each action and let each time unit of the environment be 1 minute.
    Agents cannot know the specific time of an action until performing this action. 
    Once agents perform an action (\eg, \coloredtexttt{wash cup}), the environment returns feedback for the agent (\eg, \coloredtexttt{Doing wash cup, it will take 3 times}). 
    When the action is completed, the environment returns feedback like (\eg, \coloredtexttt{cup is clean.}) and a score.
    \item \textbf{Occupancy}  
    Inspired by the observation of parallel processing, we find that the key to parallelism lies in the different states of the agents when it performs different actions.
    Therefore, we consider two action types based on whether the agent is occupied.
    One type will let agents be occupied and they cannot perform other actions until this action is completed.
    The other type will not make agents occupied so agents can engage in additional activities while performing the action.
\end{itemize}




\paragraph{Objects $\mathcal{O}$}
In \method, there are 71 different objects for all the tasks.
Every single task has an object set and there exists an overlap of object set between the two tasks in the task set.
Consistent with the occupation of action, we also consider the occupancy of every object.
The objects involved in the action are set to an occupied state when the action begins (\eg, \coloredtexttt{wash cup} will cause the object \coloredtexttt{cup} to be occupied) and agents cannot use the object while the object is occupied.
After the action is completed, they return to a non-occupied state.




\paragraph{Feedback $\mathcal{F}$}
Feedback is result following an action and related objects from the environment, including the observation of correct and incorrect inputs.

Incorrect inputs will trigger erroneous feedback in the environment.
These inputs mainly include the following types:
\begin{inparaenum}[1)]
    \item \textbf{Invalid Action:}
    The actions do not match the format required in the instruction. The environment will return the message \textit{``Invalid action''} and the whole list of valid actions.
    \item \textbf{Perform Action on Non-existing Object:}
    If the visiting objects are not in the object set, the environment will return \textit{``visiting non-existent object''} and the whole object set.
    \item \textbf{Do Not Meet Dependency:}
    When agents perform actions without completing the prerequisite actions, the feedback will contain a warning and the current state of the visiting object (\eg, \textit{``You cannot perform action \coloredtexttt{add to} on object \coloredtexttt{shrimp}. Because \coloredtexttt{shrimp} is \coloredtexttt{raw}''.})
    \item \textbf{Perform Action on Occupied Object:}
    When agents want to use occupied objects, the environment will refuse and return the reason (\eg, \textit{``Object \coloredtexttt{pot} is being occupied by another action''.})
\end{inparaenum}

Correspondingly, correct input will trigger the right feedback, which mainly contains:
\begin{inparaenum}[(1)]
    \item \textbf{Valid Action:}
    Valid action refers to the input in a valid format, and the prerequisite actions have already been completed.
    Environment will return a message containing the specific performing time, marking the start of the action (\eg, \textit{You are doing \coloredtexttt{wash cup}, it will take 9 minutes.}).
    \item \textbf{Action Completion:}
    When an action is completed,  the feedback will be the current state of the objects involved in this action (\eg, \textit{``cup is clean.''}).
\end{inparaenum}




\paragraph{Score $\mathcal{S}$}
$S$ indicates the scores from the environment ranging from 0 to 100. 
Each successfully performed action yields a score based on the action's duration and actions that take longer to complete bring larger score.
We assign score based on the action's completion time as a proportion of the total time for all actions (\eg, If completing all actions takes 15 minutes and \coloredtexttt{cook soup} takes 6 minutes, the score for completing \coloredtexttt{cook soup} is 40):
\begin{equation*}
    S_i = \frac{T_i}{\sum_{j=1}^{n} T_j} * 100
\end{equation*}
where $S_i$, $T_i$ respectively denote the score and duration of the $i$-th action. 
$n$ represents the number of all actions need to be performed.

















 


==> archived/036method_backup2.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/main.pdf}
    \caption{An overview of \method, with an multitasking example that shows our designs of the simulation. 
    \method first set an objective for the agent and then the agent interacts with \method over time, with the design of task dependency, object occupancy and agent occupancy.}
    \label{fig:TimeArena}
\end{figure*}

In this paper, we create \method, a text-based simulated environment to evaluate the effcient multitasking capabilities of language agents.
To help illustrate, we first show an overview and an example run of how an agent interacts with the \method environment ($\mathsection$~\ref{sec3:overview}), and then describe the design of the simulation environment in more detail ($\mathsection$~\ref{sec3:components}-\ref{sec3:feedback}).



\subsection{Overview of \method}
\label{sec3:overview}









\method challenges agents to complete multiple tasks strategically in the shortest possible time. 
This simulation emphasizes the importance of understanding, performing, and optimizing actions within a constrained timeframe, mirroring practical scenarios of time management.

Central to \method are \textbf{Tasks}, \textbf{Objects}, and \textbf{Actions}. \textbf{Tasks} define the objectives for the agents, \textbf{Objects} represent elements in the environment that agents will encounter and interact with, and \textbf{Actions} are the means to accomplish these tasks. 
Real-time feedback and scoring mechanisms are integral to the environment, assessing agent performance and adding to the simulation's complexity and realism. 
Unique features like the duration and occupancy of actions, and strategic resource utilization, distinguish \method from other environments.

\paragraph{An Example Run}
As in Figure~\ref{fig:TimeArena}, consider an agent tasked with ``make tea'' (Task 1), ``wash clothes'' (Task 2) and ``wash bed sheet'' (Task 3).
The agent starts by decomposing the task into actions like \coloredtexttt{boil water}.
In \method, all actions have duration (\eg, \coloredtexttt{Boil water} needs 8 minutes.) and dependencies (\eg, At T=4min, \coloredtexttt{make tea} violates the dependency because \coloredtexttt{wash teapot} and \coloredtexttt{boil water} are not completed yet.).
The agent then interacts with objects (e.g., \coloredtexttt{wash clothes in washing machine}) which become \textbf{occupied} during the process. 
The agent can engage in non-occupied
actions simultaneously (e.g., \coloredtexttt{wash teapot}) while others (e.g., \coloredtexttt{boil water}) are in progress.
Environmental feedback guides the agent, indicating the legitimacy of actions and the completion of tasks. 
For example, if the \coloredtexttt{washing machine} is occupied, the agent adjusts its strategy. 
The agent's goal is to complete all tasks efficiently, with performance evaluated based on progress and completion time.

This dynamic interaction in \method fosters an environment where strategic planning, resource management, and adaptability are key to an agent's success.

 


\subsection{Components of \method}
\label{sec3:components}

\paragraph{Tasks}
In \method, We design tasks within three distinct \textit{scenarios} or simulated settings, namely, \textit{household activities}, \textit{cooking}, and \textit{laboratory work}.
Each scenario represents a specific context or environment where multitasking is an integral part of the activities involved.\footnote{Details of tasks are in Appendix~\ref{app:task}.}
For example, one can do a \coloredtexttt{sweep floor} while doing \coloredtexttt{boil water}, and do a \coloredtexttt{wash dishes} while doing \coloredtexttt{cook soup}.
Each scenario contains several tasks (\eg, 10), and actions and objects are shared across multiple tasks of a scenario.
Each task requires multiple actions to be executed, which manipulates the objects in the environment for task completion.
In the beginning, \method gives a list of tasks to the agent, with a comprehensive task instruction consisting of a \textit{task description}, an \textit{action space}, and an \textit{object set}:
\begin{itemize}[noitemsep]
    \item \textbf{Task Description}: Introduces task objectives (\eg, ``Task 1: Make a dish of beef fried rice, which consists of cooked rice and fried beef.'');
    \item \textbf{Action Space}: List the valid actions for the tasks (\eg, \coloredtexttt{chop}, \coloredtexttt{wash});
    \item \textbf{Object Set}: List the available objects in the environment for the tasks (\eg, \coloredtexttt{pot}, \coloredtexttt{beaker}).
\end{itemize}
At every timestep $t$, the agent needs to perform valid actions on the objects, and receives feedback from the environment.

\paragraph{Objects}
Objects are integral to completing tasks, situating within the environment.
In \method, there are 71 different objects for all the tasks.
Every task involves a list of objects, which might overlap with other tasks of the same scenario.
To mimic the resource limitation in real world parallel processing, we introduce:
\begin{itemize}
    \item \textbf{Object Occupancy}: the state of the object involved in an action is set to be \textit{occupied}, \eg, \coloredtexttt{wash cup} will cause the object \coloredtexttt{cup} to be occupied.
    This object cannot be processed until the involving action is completed (after some time).
    Then, this object is reset as non-occupied and waits for another action.
\end{itemize}



\paragraph{Actions}

We design a total of 45 actions for all 30 tasks.
Each action consists of a detailed description (\eg, \coloredtexttt{chop OBJ}, \coloredtexttt{chop the whole item into sliced pieces.}), showing a change of states the action will cause to an object.\footnote{All the actions are listed in Apendix~\ref{app:action}.}
Different from existing text-based simulations~\cite{wang-etal-2022-scienceworld,gong2023mindagent,shridhar2020alfworld}, in our case, an action has a duration of time and may occupy the agent from performing other actions, to the passage of time.
In detail:
\begin{itemize}[noitemsep]
    \item \textbf{Action Dependency}: An action within the same task might be dependent on the completion of other actions within the same task. 
    As depicted in Figure~\ref{fig:TimeArena}, \coloredtexttt{make tea} is dependent on \coloredtexttt{wash teapot}.
    \item \textbf{Duration of Time}:
    Each action holds a timeframe in the timeline, ranging from 1 to 10 minutes.
    In practice, agents only have an educated guess of the time duration of each action until actually interacting with \method.  
    \item \textbf{Agent Occupancy}:  
    One key to parallel processing is agent occupancy that prevents agents from performing other tasks.
    Therefore, we consider two types of actions based on agent occupancy:
    1) Type 1 action occupies the agent til completion (\eg, \coloredtexttt{wash teapot}); and 2) Type 2 action lets agents be idle, allowing to perform other actions (\eg, \coloredtexttt{boil water}).
\end{itemize}


\subsection{Agent Interaction and Environmental Feedback}
\label{sec3:feedback}
\paragraph{Environmental Feedback}
The feedback from a textual environment is important to simulate and implement the constraints in \method using only textual message.
We define feedback as the response from the environment following an action by an agent.
A feedback message could be of multiple types, including:
\begin{itemize}[noitemsep]
    \item \textbf{Invalid Action}:
    An action attempt that does not match the required format, \eg, \textit{``\coloredtexttt{clean teapot} is invalid''}.
    \item \textbf{Acting on Non-existing Object}:
    An action attempt that visits objects that are not in the object set, \eg, \textit{``\coloredtexttt{pan} is non-existent''}.
    \item \textbf{Wrong Action Input}:
    An action attempt that the prerequisite action has not completed (\eg, \textit{``Cannot perform action \coloredtexttt{add to} on object \coloredtexttt{shrimp}. Because \coloredtexttt{shrimp} is \coloredtexttt{raw}''.}) or has been completed (\eg, \textit{``\coloredtexttt{wash beaker} has been completed''}).
    \item \textbf{Action not Match Object}:
    An action attempt that does not match the object, \eg, \textit{``You cannot perfrom \coloredtexttt{wash} on \coloredtexttt{potato}.''}\kyle{I'm confused by this example, does it say that washing a potato is not a valid or possible action? If so, perhaps there's a better example of an invalid action given that washing a potato is normal in the real world}
    \item \textbf{Action on Occupied Object}:
    An action attempt on occupied objects, \eg, \textit{``Object \coloredtexttt{pot} is being occupied by another action''.}
\end{itemize}
Correspondingly, valid actions will trigger environmental feedback of the following types:
\begin{itemize}[noitemsep]
    \item \textbf{Action Start}:
    Avoiding previous errors,
    valid actions will receive a feedback message containing the specific performing time, marking the start of the action, \eg, \textit{You are doing \coloredtexttt{wash cup}, it will take 9 minutes}.
    \item \textbf{Action Completion}:
    When an action is completed, the environment will send a message, \eg, \coloredtexttt{cup is clean}, and reset the occupying state of the object (\coloredtexttt{cup}).
\end{itemize}


\paragraph{Progress Score}
The environment also records the progress score (\%) of the agent.
Take the amount of time to complete all actions as 100\% of its full time.\kyle{(i.e., the denominator below, right?)}
Each successfully performed action contributes to the progress score based on its time duration.
Formally, an action takes up $t_i$ minutes\kyle{is this the time of the action independently, or after other things have happened? I'm still confused. Suppose action $t_{1}$ takes 5 second and the full time for all actions takes $20$ seconds, so $s_{1} = 0.25$. Now let's say that action at $t_{2} = 5$ seconds again, so $s_{2} = 0.25$? How does this show progress, I'm missing something still. If $t_{1} = 10$, then this makes sense, but hard to understand this from the description and equation}, so the completion of it contributes to a progress score $s_i = \frac{t_i}{\sum_{j=1}^{n} t_j} * 100\%$,
where $n$ is the number of all required actions.


==> archived/040experi_2_7_backup.tex <==

\input{table/env_statistic}
\subsection{Experiment Settings}



\paragraph{Task Set Construction}
In our experiments, we design three categories of task combinations based on the number of tasks: \textbf{\# Task=1}, \textbf{\# Task=2} and \textbf{\# Task=3} scenarios.
In \# Task=1 scenario, agents focus on completing one task (\eg, \textit{make tea}).
For the other two scenarios, we combine either two or three tasks from 10 single tasks (\eg, \textit{make tea and wash clothes}).
Then, we randomly select 10 combined tasks for each scenario.\footnote{Appendix~\ref{app:example} shows examples of single tasks and combined tasks.}




\paragraph{Interaction}
Initially, the environment provides a comprehensive task instruction that details the task, action space, and object set. 
Subsequently, the agent produces an action based on this instruction, adhering to a prescribed format specified in the action space; any deviation is considered invalid. 
To facilitate action recognition by the environment, regular expressions are employed to parse actions from responses (e.g., extracting \textit{wash clothes} from \textit{"I will wash clothes''}). 
For each action execution, the agent must incorporate task instructions, previous actions, and feedback from the environment into the language model as context.
\footnote{Appendix~\ref{app:example} shows an example of interaction between agent and environment.}

\kyle{In these examples its not clear how the model specifies that two things can be done at once, how does it do actually operationalize parallel processing? Also,  an example with wait would be helpful in the appendix, I'm still a little unclear what the model does with this command.}


\paragraph{Maximum Time}
Each combined task is allocated a maximum completion time.
We set the time limit for completing a single task at 40 minutes, which exceeds the total time required for all actions in any given task. 
For tasks that are combined, the time limit is proportionally increased by the number of tasks involved.



\paragraph{Oracle Performance}
As shown in Tabel~\ref{tab:main}, \textit{Orcale} represents the optimal performance, including the shortest completion time and the fastest completion rate, which are manually calculated.
\zyk{Specifically, we calculate oracle performance using a greedy strategy: always start the longest non-occupied actions as early as possible.}
\cjj{add an algorithm in the Appendix.}

\input{table/main_exp}
\paragraph{Finishing}
The interaction finishes under any of the following conditions:
\begin{inparaenum}[(1)]
    \item 
    Agents have completed all the actions that solve the tasks
    (\ie, the progress score reaches 100\%)
    \item The time has run out;
    \item The agents have performed incorrect actions 5 times in a row are considered to have failed the task.
\end{inparaenum}



\paragraph{Model Choice}
We select a variety of language models to drive the agent: Mistral-7B~\cite{jiang2023mistral} by MistralAI, OpenChat-3.5~\cite{wang2023openchat} which is fine-tuned from a 7B Mistral model fine-tuned with C-RLFT (\texttt{openchat\_3.5}), Vicuna-13B~\cite{chiang2023vicuna} which is fine-tuned from a 13B LLaMA model~\cite{touvron2023llama} with instructions and user-shared conversations, Mixtral-8x7B~\cite{mistralai_2023_mixtral} by MistralAI, which is a Mixture-of-Expert version of Mistral, Gemini Pro by Google~\cite{team2023gemini}, GPT-3.5~\citep{openai2022chatgpt} by OpenAI (\texttt{gpt-3.5-turbo-1106}) and GPT-4~\citep{openai2023gpt4} by OpenAI (\texttt{gpt-4-1106-preview}).

\begin{figure}[t]
    \centering    
    \includegraphics[width=\linewidth]{figure/error.pdf}
    \caption{The proportions of correct and incorrect actions of each language agent.
    }
    \label{fig:error}
\end{figure}

     







\subsection{Evaluation Metrics}
To comprehensively evaluate the ability of agents to multitask, we consider both time and score and design the following four metrics:
\begin{itemize}
    \item \textbf{Average Progress Score (score, AS)}: The average highest progress score achievable by an agent:
            \begin{equation*}
                AS = \frac{\sum_{i \in N} P_i}{N}
            \end{equation*}
        where $P_i$ denotes the maximum progress score of $i$-th task that agents can reach, and $N$ denotes the number of all tasks.  
    \item \textbf{Completion Speed (score per minute, CS)}: The average of the highest score divided by the time taken to achieve it:
        \begin{equation*}
            CS = \frac{\sum_{i \in N} P_i}{\sum_{i \in N} T_i}
        \end{equation*}
    where $T_i$ denotes the time required to reach $P_i$ of $i$-th task.
    \item \textbf{Task Completion Rate (\%, CR)}: The rate of successfully completed tasks:
        \begin{equation*}
            CR = \frac{S}{N}
        \end{equation*}
    where $S$ denotes the tasks completed successfully.
    Notably, when combining tasks, a combined task counts as one task.
    \item \textbf{Average Completion Time (minutes, CT)}: The average time taken for completing tasks successfully:
        \begin{equation*}
            CT = \frac{\sum_{i \in S} T_i}{S}.
        \end{equation*}
\end{itemize}






\subsection{Main Results}

Based on the performance of language agents in Table~\ref{tab:main}, GPT-4 achieves the best performance across different task combinations. 
Moreover, the combined tasks are more challenging than single tasks despite the longer time given.
Apart from GPT-4, most models fail to complete 2 or 3 tasks, showing their limited multitasking abilities and the challenging nature of our environment.

For open-source models, OpenChat-3.5 and Vicuna-13B are even better than GPT-3.5, demonstrating the potential of open-sourced models to develop multitasking capabilities.
However, although OpenChat-3.5 and Vicuna-13B exhibit faster completion speed and shorter average completion time than GPT-4, a lower task completion rate indicates that these models quickly complete simple actions initially but then encounter difficulties;
they either get caught in repetitive actions or fail to properly segment subsequent tasks, which significantly impacts task performance.
For example, initially, \coloredtexttt{potato} is unpicked, so the agent first performs \coloredtexttt{pick potato}. 
Subsequently, the agent mistakenly opts for \coloredtexttt{cook potato in pot} rather than the correct \coloredtexttt{chop potato}, because it incorrectly decomposes the task.


To explore the potential of heuristic algorithms in improving model performance, we introduce self-plan prompting to GPT-4, as illustrated in Appendix~\ref{app:example}. This method necessitates that the model initially discerns the dependencies among actions, task descriptions, and objects, and estimates the duration of each action. It then adopts a greedy strategy akin to Oracle Performance, favoring the selection of the longest duration actions that do not require continuous engagement from the agent in the task model to formulate a plan. Then, the agent executes this plan through interactions with the environment.
The results indicate that self-plan prompting is outperformed by the vanilla GPT-4. 
This is due to the model's difficulty inaccurately parsing actions and identifying their dependencies. 
Additionally, the model's reliance on estimating action durations might introduce cascading errors, leading to inaccurate results of the greedy strategy.
Moreover, the model's rigid adherence to flawed plans, without adapting to the dynamic nature of interactions with the environment, leads to its failure.


\subsection{Analysis}



\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/constraint.pdf}
    \caption{Comparison of the performance of GPT-4 with and without resource constraints. 
    We imposed constraints by limiting to a single instance each of \coloredtexttt{pot}, \coloredtexttt{fryer}, and \coloredtexttt{oven}.
    }
    \label{fig:constraint}
\end{figure} 


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/reward_curve.pdf}
    \caption{
    Task progress score curves of language agents on two task combinations in \method. %Each subfigure displays the progress score obtained by the agent over time.
    The names at the bottom-right indicate the scenario and task number. 
    For example, \texttt{cooking1} represents the first combination of tasks in the cooking scenario.
    }
    \label{fig:progress}
\end{figure*}

\paragraph{Can language agents master multitasking?}
To further explore whether language agents can master multitasking, we conduct detailed analyses to investigate the types of actions these models can perform.
Based on environmental feedback, the actions are classified into two categories: correct ones and incorrect ones.
We further define six fine-grained types of actions:
1) \textbf{Correct Actions}: Valid Action, Wait
2) \textbf{Incorrect Actions}: Invalid Action/Object, Dependency Violation, Repeating Completed Action and Object-Mismacthed Action.\footnote{Detailed description of different types of actions can be found in Appendix~\ref{app:actiontype}.}

We calculate the frequency of these actions of each agent throughout their interactions.
The results in Figure~\ref{fig:error} show that a significant proportion of invalid actions are due to dependency violations and mismatches with objects.
Multitasking involves performing several tasks simultaneously. 
As the number of tasks increases, the complexity of objects and actions escalates, leading to intricate dependencies between actions.
Thus, the high proportion of actions that violate dependencies and mismatch objects suggests that language agents face challenges in managing complex action interdependencies during multitasking, indicating a limitation in their multitasking capabilities.

\paragraph{Are language agents aware of parallel processing?}
Parallel processing can significantly reduce the time required for efficient multitasking. 
As stated in $\mathsection$~\ref{sec3:components}, we consider the duration of time for each action in \method to explore the parallel processing capabilities of language agents.
If an agent is capable of parallel processing, it can engage in additional actions instead of unnecessary waiting for the current action to complete.
To answer this question, we decompose \coloredtexttt{wait} action into two types: \coloredtexttt{necessary wait} and \coloredtexttt{unnecessary wait}.
The former represents that no actions can be performed currently, requiring the wait for other actions to complete. 
In particular, we report the maximum number of \coloredtexttt{necessary wait}. 
\coloredtexttt{Unnecessary wait} indicates that there are other action options available.
Figure~\ref{fig:error} shows that \coloredtexttt{wait} actions constitute over half of the valid actions performed by different LLMs, and \coloredtexttt{necessary wait} only accounts for a small part of it.
This indicates a tendency for agents to engage in unnecessary waiting, showing their ignorance of parallel processing and inability of completing tasks in minimal time (Table~\ref{tab:main}).








\paragraph{Do resource constraints affect the multitasking of language agents?}
Resource constraints refer to limitations in the availability of resources (\eg, the number of objects) necessary for task completion, which is rather common in real life.
To design resource constraints, we first select three objects: \coloredtexttt{pot}, \coloredtexttt{fryer} and \coloredtexttt{oven} in the cooking scenario, and choose \# Task=2 setting in Table~\ref{tab:main}.
Then, we set that there is only one instance of each of the three objects, simulating the limitation of resources in the environment.
Figure~\ref{fig:constraint} compares GPT-4's performance before and after applying these constraints. 
We find that the constraints do not affect the task completion time or speed, revealing that GPT-4 rarely attempts to process tasks in parallel.
However, a noticeable decline in both completion rate and progress score indicates that the constraints prevent the models from better comprehending and decomposing multiple tasks.








\paragraph{Language agents trapped in an infinite loop.}
To delve into the reason language agents struggle with multiple tasks, we analyze the progress score changes over time for various models.
As illustrated in Figure~\ref{fig:progress}, Vicuna, Mistral, Gemini and GPT-3.5 often cease scoring without completing all tasks, maintaining low scores until time runs out (\eg, (5,b), (2,c) and (6,d)).
We further examine their actions during these periods and find that they always perform \textbf{incorrect actions and waiting} alternately.
Since \coloredtexttt{wait} is a valid action, repeatedly alternating between waiting and incorrect actions does not lead to task failure, but neither does it contribute to an increase in scores.
To find out whether agents wait for the good reasons, we ask them to explain for each action via chain-of-thought, and they often believe \coloredtexttt{wait} can pause incorrect actions.
However, they find it hard to adjust their incorrect actions based on feedback after waiting, resulting in them being trapped in infinite loops.




==> archived/040experiment.tex <==


\subsection{Interaction Settings}


\input{table/main_exp}




Based on 30 tasks, we set up the entire experiment to evaluate language agents on \method. 
The detailed settings of interaction are introduced as follows:

\paragraph{Task Set Construction}
In our experiment, we design three categories of task combinations: \ie, single-task, two-task and three-task scenarios.
In single-task scenario, language agents focus on actions within one task, striving for speedy completion.
For the two-task and three-task categories, in each scenario, we combine either two or three single tasks from a pool of ten single tasks.
Then, we randomly select 10 combined tasks for each of these scenarios in the task set.


\paragraph{History}
For each interaction, the history comprises a sequence of dialogues. 
This includes the initial instructions from the environment, the agent's actions, and the environment's feedback. 
These elements are spliced together across multiple rounds to form the interaction history that needs to be inputted.



\paragraph{Action Parsing}
Initially, the model must produce outputs in a specific format as outlined in the instructions. 
Any action that deviates from this format is invalid in the environment. 
Additionally, we also adopt some regular expressions to extract actions from responses for agents, ensuring they are interpretable by the environment.


\paragraph{Maximum Time}
Each combined task is allocated a maximum duration. 
We set the time limit for completing a single task at 40 minutes, which exceeds the total time required for all actions in any given task. 
For tasks that are combined, the time limit is proportionally increased by the number of tasks involved.


\paragraph{Finishing}
The interaction finishes under any of the following conditions:
\begin{inparaenum}[(1)]
    \item Agents complete all the tasks (\ie, the score accumulates to 100); 
    \item The time has run out;
    \item The agents perform incorrect actions five times in a row and are considered to have failed the task.
\end{inparaenum}


\paragraph{Language Agents}
We select a variety of language models to drive the agent and record the interaction trajectories between the agent and the environment: Mistral-7B~\cite{jiang2023mistral} by MistralAI, OpenChat-3.5~\cite{wang2023openchat} which is fine-tuned from a 7B Mistral model fine-tuned with C-RLFT (\texttt{openchat\_3.5}), Vicuna-13B~\cite{chiang2023vicuna} which is fine-tuned from a 7B LLaMA model~\cite{touvron2023llama} with instructions or user-shared conversations, Mixtral-8x7B~\cite{mistralai_2023_mixtral} by MistralAI, which is a Mixture-of-Expert version of Mistral, GPT-3.5-Turbo~\citep{openai2022chatgpt} by OpenAI (\texttt{gpt-3.5-turbo-1106}) and GPT-4~\citep{openai2023gpt4} by OpenAI (\texttt{gpt-4-1106-preview}).

      
\input{table/env_statistic}







\subsection{Evaluation Metric}
To comprehensively evaluate the ability of agents to perform multi-task planning, we consider both time and score dimensions and design the following four metrics:
\begin{itemize}
    \item \textbf{Average Score (score, AS)}: The average highest score achievable by an agent.
            \begin{equation*}
                AS = \frac{\sum_{i \in N} P_i}{\lvert N \rvert}
            \end{equation*}
        where $P_i$ denotes the maximum score of $i$-th task that agents can reach.
        
    \item \textbf{Completion Velocity (score per minute, CV)}: The average of the highest score divided by the time taken to achieve it.
        \begin{equation*}
            CV = \frac{\sum_{i \in \lvert N \rvert} \frac{S_i}{T_i}}{\lvert N \rvert}
        \end{equation*}
    where $S_i$ denotes the maximum score of $i$-th task and $T_i$ denotes the time required to reach $S_i$ of $i$-th task.
        
    \item \textbf{Task Completion Rate (\%, CR)}: The rate of successfully completed tasks.
        \begin{equation*}
            CR = \frac{\lvert S \rvert}{\lvert N \rvert}
        \end{equation*}
    where $S$ denotes the tasks completed successfully and $N$ denotes all the tasks.
    Notably, when combining tasks, a combined task counts as one task.
    
    \item \textbf{Average Completion Time (minutes, CT)}: The average time taken for completing tasks successfully.
        \begin{equation*}
            CT = \frac{\sum_{i \in \lvert S \rvert} T_i}{\lvert S \rvert}
        \end{equation*}
    where $T_i$ represents the time of $i$-th successfully completed task.
\end{itemize}







\subsection{Main Results}
We report the performance of language agents in Table~\ref{tab:sta} with different task combination settings.
Based on the results, we find that GPT-4 achieves the best performance across different task combinations. 
However, there is still room for enhancement in cooking and laboratory contexts.
Moreover, the horizontal comparison reveals that combined tasks are more challenging than single tasks despite the longer time given.
Apart from GPT-4, most models fail to complete two or three tasks, highlighting their limited multitasking abilities and the challenging nature of our environment.

For open-source models, OpenChat-3.5 and Vicuna-13B even perform better than GPT-3.5-Turbo, demonstrating their potential to develop multitasking capabilities.
However, although OpenChat-3.5 and Vicuna-13B exhibit faster completion speeds and shorter average completion times than GPT-4, a lower task completion rate indicates that these models can quickly complete simpler actions initially but then encounter difficulties.
They either get caught in repetitive actions or fail to properly segment subsequent tasks, significantly impacting their performance.











\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/constraint.pdf}
    \caption{Comparison of the performance of GPT-4 on AS, CV, CR and CT with and without constraints.}
    \label{fig:constraint}
\end{figure}



\begin{figure}[!b]
    \centering    
    \includegraphics[width=\linewidth]{figure/error.pdf}
    \caption{Statistics of action proportions of different models. \textit{Invalid Action/Object} represents an action that does not conform to the format (\eg, the valid action is \coloredtexttt{sweep floor}, but the model chooses \coloredtexttt{clean floor}.) or an object that does not exist (\eg, \coloredtexttt{fry beef in pan} but \coloredtexttt{pan} is not in the object set); \textit{Repeat Completed Action} represents an action is valid but has been completed (\eg, performing \coloredtexttt{sweep floor} twice); \textit{Violate Dependency} means that the action does not meet the prerequisites (\eg, \coloredtexttt{make tea} before \coloredtexttt{washing teapot}); \textit{Not Match Object} means that the action does not match the object (\eg, \coloredtexttt{beef} needs \coloredtexttt{fry} but \coloredtexttt{cook}.); \textit{Valid Action} means correct actions and \textit{wait} means that the agent chooses to wait for one minute.}
    \label{fig:error}
\end{figure}

\subsection{Analysis \& Discussion}

\paragraph{Scheduling for Multiple Tasks with Resource Constraints}
Resource constraints refer to limitations in the availability of resources (\eg, the number of objects) necessary for task completion.
In examining the effects of object quantity on multitasking scheduling for language agents, we first select three objects: \coloredtexttt{pot}, \coloredtexttt{fryer} and \coloredtexttt{oven} in the cooking scenario.
Then, we choose two-task settings of the cooking scenario in Table~\ref{tab:main} and set the above three objects to appear only once at most as constraints.
Figure~\ref{fig:constraint} displays a comparison of GPT-4's performance before and after applying these constraints. 
The findings show that the constraints do not alter the task completion time or velocity, revealing that GPT-4 rarely attempts to process tasks in parallel.
However, a noticeable decline in both completion rate and rewards indicates that the constraints hinder the model's ability to comprehend and decompose multiple tasks.








\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/reward_curve.pdf}
    \caption{We show the score changes over time of \textcolor[rgb]{0.99,0.75,0.52}{Mistral-7B}, \textcolor[rgb]{0.45,0.43,0.70}{Vicuna-13B}, \textcolor[rgb]{0.10,0.62,0.47}{GPT-3.5-turbo}, and \textcolor[rgb]{0.84,0.11,0.11}{GPT-4} in the two-task setting. The x-axis represents time and the y-axis represents progress score.}
    \label{fig:progress}
\end{figure*}





\paragraph{The Impart of \textit{Wait} on Completing Tasks}
Figure~\ref{fig:progress} illustrates the agent's cumulative score over time. 
A flat curve segment, showing no increase, indicates that the agent is continuously engaged in trial-and-error processes and waiting.
Since \coloredtexttt{wait} is recognized as a valid action, repeatedly alternating between waiting and incorrect actions does not lead to task failure. 
Notably, Vicuna, Mistral, and GPT-3.5-turbo models often enter a loop of trial-and-error and waiting.
We analyse that these models anticipate changes in object states through waiting, hoping to enable otherwise unfeasible actions.
For example, the agent choose \coloredtexttt{wait} for several minutes during \coloredtexttt{cook beef}.
Then the agent strongly believes that by waiting, a change in the state will occur.
So when performing invalid actions and trigger an error from environment, the agent expects that while waiting, there will be a state change which allows the invalid action to be performed successfully. 
This reveals the models' imprecise understanding of the environment's dynamic state changes over time. 
Moreover, the model has a deep belief in this situation and usually falls into an infinite loop, making it difficult to modify its beliefs based on feedback.








\paragraph{Dependency Among Actions Across Different Tasks}

Dependencies are concealed within an object's state and the changes that actions can induce. 
As the number of tasks grows, so does the complexity of the objects, actions, and their interdependencies. 
Figure~\ref{fig:error} reveals that a significant number of invalid actions are due to actions that disregard these dependencies. 
This suggests that language agents have difficulty considering an object's current status and past actions when breaking down tasks and carrying out actions.

Additionally, Table~\ref{tab:main} shows a steep drop in the language agents' task completion rates as the number of tasks increases. 
This trend indicates that the agents tend to try complete several tasks, leading to interference between tasks. 
Such confusion results in the agent's misunderstanding of the current status of the object and the goals of task 1, causing it to fail.
For example, at time t, while planning the next step for task 1, the agent could incorrectly consider history from task 2. For instance, ``make fried rice'' might require \coloredtexttt{add potato}, while ``make noodles'' does not. Yet, the agent might end up doing \coloredtexttt{mix potato and noodles} due to interference from the other task.



\paragraph{Awareness of Parallel Processing}
The agent's decision-making process is mirrored in its choice of actions. 
In \method, we distinguish between two action types based on agent occupancy. 
Our findings indicate that language agents prefer waiting when they are unoccupied and no object state changes. 
As shown in Figure~\ref{fig:error}, 90.9\% of GPT-4's actions are valid, with CR and AS nearing perfect scores (Table~\ref{tab:main}). 
Yet, gaps in CT and CV compared to the fastest completion time exist. 
Interestingly, half of GPT-4's effective actions are waits, suggesting repeated waiting post-task completion. 
The model opts to wait for object state changes rather than processing tasks in parallel. 
In \method, tasks contain both parallel (independent) and serial (dependent) actions. 
The model’s tendency to avoid switching to other tasks while executing a serial task chain highlights a crucial aspect for multitasking and parallel processing.



==> archived/041expsetup.tex <==


\subsection{Interaction Settings}
\input{table/env_statistic}






Based on 30 tasks, we set up the entire experiment to evaluate language agents on \method. 
The detailed settings of interaction are introduced as follows:

\paragraph{Task Set Construction}
In our experiment, we design three categories of task combinations: \ie, single-task, two-task and three-task scenarios.
In single-task scenario, language agents focus on actions within one task, striving for speedy completion.
For the two-task and three-task categories, in each scenario, we combine either two or three single tasks from a pool of ten single tasks.
Then, we randomly select 10 combined tasks for each of these scenarios in the task set.


\paragraph{History}
For each interaction, the history comprises a sequence of dialogues. 
This includes the initial instructions from the environment, the agent's actions, and the environment's feedback. 
These elements are spliced together across multiple rounds to form the interaction history that needs to be inputted.



\paragraph{Action Parsing}
Initially, the model must produce outputs in a specific format as outlined in the instructions. 
Any action that deviates from this format is invalid in the environment. 
Additionally, we also adopt some regular expressions to extract actions from responses for agents, ensuring they are interpretable by the environment.


\paragraph{Maximum Time}
Each combined task is allocated a maximum duration. 
We set the time limit for completing a single task at 40 minutes, which exceeds the total time required for all actions in any given task. 
For tasks that are combined, the time limit is proportionally increased by the number of tasks involved.


\paragraph{Finishing}
The interaction finishes under any of the following conditions:
\begin{inparaenum}[(1)]
    \item Agents complete all the tasks (\ie, the score accumulates to 100); 
    \item The time has run out;
    \item The agents perform incorrect actions five times in a row and are considered to have failed the task.
\end{inparaenum}


\paragraph{Language Agents}
We select a variety of language models to drive the agent and record the interaction trajectories between the agent and the environment: Mistral-7B~\cite{jiang2023mistral} by MistralAI, OpenChat-3.5~\cite{wang2023openchat} which is fine-tuned from a 7B Mistral model fine-tuned with C-RLFT (\texttt{openchat\_3.5}), Vicuna-13B~\cite{chiang2023vicuna} which is fine-tuned from a 7B LLaMA model~\cite{touvron2023llama} with instructions or user-shared conversations, Mixtral-8x7B~\cite{mistralai_2023_mixtral} by MistralAI, which is a Mixture-of-Expert version of Mistral, GPT-3.5-Turbo~\citep{openai2022chatgpt} by OpenAI (\texttt{gpt-3.5-turbo-1106}) and GPT-4~\citep{openai2023gpt4} by OpenAI (\texttt{gpt-4-1106-preview}).

      








\subsection{Evaluation Metric}
To comprehensively evaluate the ability of agents to perform multi-task planning, we consider both time and score dimensions and design the following four metrics:
\begin{itemize}
    \item \textbf{Average Score (score, AS)}: The average highest score achievable by an agent.
            \begin{equation*}
                AS = \frac{\sum_{i \in N} P_i}{\lvert N \rvert}
            \end{equation*}
        where $P_i$ denotes the maximum score of $i$-th task that agents can reach.
        
    \item \textbf{Completion Velocity (score per minute, CV)}: The average of the highest score divided by the time taken to achieve it.
        \begin{equation*}
            CV = \frac{\sum_{i \in \lvert N \rvert} \frac{S_i}{T_i}}{\lvert N \rvert}
        \end{equation*}
    where $S_i$ denotes the maximum score of $i$-th task and $T_i$ denotes the time required to reach $S_i$ of $i$-th task.
        
    \item \textbf{Task Completion Rate (\%, CR)}: The rate of successfully completed tasks.
        \begin{equation*}
            CR = \frac{\lvert S \rvert}{\lvert N \rvert}
        \end{equation*}
    where $S$ denotes the tasks completed successfully and $N$ denotes all the tasks.
    Notably, when combining tasks, a combined task counts as one task.
    
    \item \textbf{Average Completion Time (minutes, CT)}: The average time taken for completing tasks successfully.
        \begin{equation*}
            CT = \frac{\sum_{i \in \lvert S \rvert} T_i}{\lvert S \rvert}
        \end{equation*}
    where $T_i$ represents the time of $i$-th successfully completed task.
\end{itemize}







==> archived/046experiment_backup.tex <==

\input{table/env_statistic}
\subsection{Experiment Settings}
\input{table/main_exp}


\paragraph{Task Set Construction}
In our experiments, we design three categories of task combinations based on the number of tasks: \textbf{\# Task=1}, \textbf{\# Task=2} and \textbf{\# Task=3} scenarios.
In \# Task=1 scenario, agents focus on completing one task.
For the other two scenarios, we combine either two or three tasks from 10 single tasks.
Then, we randomly select 10 combined tasks for each scenario.\footnote{Appendix~\ref{app:example} shows examples of single tasks and combined tasks.}\kyle{this is very confusing. Maybe an example here can help. ``In .. agent focus on completing one task (e.g., EXAMPLET ASK).. For the other two scenarios we combined with two or three tasks (e.g., EXAMPLE)'' }


\paragraph{History}
The history includes the initial instruction from the environment, the agent's actions, and the environment's feedback. 
When interacting with \method, the history need\kyle{needs?} to be input to the language model\kyle{see comment below. The language model here comes out of nowhere, this is first time you mention it in relation tot he environment} and then it generates the action.



\paragraph{Action Parsing}
The model must generate actions in a valid format as outlined in the instructions.\kyle{This is the first time that you are mentioning models generating things and its a bit confusing. It might make sense to start section 4 (before 4.1) just saying clearly what the setting is: ``In broad outlines, model are provided with X and must produce Y (I'm a little confused about what X and Y are exactly to be honest).. in this section we detail how the tasks are set up, the history is constructed for constructing prompts, how the models outputs are parsed...''}
Any action that deviates from this format is regard as invalid. 
Additionally, we also adopt some regular expressions to extract actions from responses to ensure they are interpretable by the environment.


\paragraph{Maximum Time}
Each combined task is allocated a maximum duration. 
We set the time limit for completing a single task at 40 minutes, which exceeds the total time required for all actions in any given task. 
For tasks that are combined, the time limit is proportionally increased by the number of tasks involved.


\paragraph{Finishing}
The interaction finishes under any of the following conditions:
\begin{inparaenum}[(1)]
    \item Agents have completed all the tasks (\ie, the progress score accumulates to 100)\kyle{all the tasks, or all the actions that solve the task? So it does go to 100\%, clears up some confusion from above}; 
    \item The time has run out;
    \item The agents have performed incorrect actions 5 times in a row are considered to have failed the task.
\end{inparaenum}


\paragraph{Model Choice}
We select a variety of language models to drive the agent: Mistral-7B~\cite{jiang2023mistral} by MistralAI, OpenChat-3.5~\cite{wang2023openchat} which is fine-tuned from a 7B Mistral model fine-tuned with C-RLFT (\texttt{openchat\_3.5}), Vicuna-13B~\cite{chiang2023vicuna} which is fine-tuned from a 13B LLaMA model~\cite{touvron2023llama} with instructions and user-shared conversations, Mixtral-8x7B~\cite{mistralai_2023_mixtral} by MistralAI, which is a Mixture-of-Expert version of Mistral, GPT-3.5~\citep{openai2022chatgpt} by OpenAI (\texttt{gpt-3.5-turbo-1106}) and GPT-4~\citep{openai2023gpt4} by OpenAI (\texttt{gpt-4-1106-preview}).

      








\subsection{Evaluation Metric}
To comprehensively evaluate the ability of agents in multitasking, we consider both time and score and design the following four metrics:
\begin{itemize}
    \item \textbf{Average Progress Score (score, AS)}: The average highest progress score achievable by an agent.
            \begin{equation*}
                AS = \frac{\sum_{i \in N} P_i}{N}
            \end{equation*}
        where $P_i$ denotes the maximum progress score of $i$-th task that agents can reach and $N$ denotes the number of all tasks.  
    \item \textbf{Completion Speed (score per minute, CV)}: The average of the highest score divided by the time taken to achieve it.
        \begin{equation*}
            CV = \frac{\sum_{i \in N} P_i}{\sum_{i \in N} T_i}
        \end{equation*}
    where $T_i$ denotes the time required to reach $P_i$ of $i$-th task.
    \item \textbf{Task Completion Rate (\%, CR)}: The rate of successfully completed tasks.
        \begin{equation*}
            CR = \frac{S}{N}
        \end{equation*}
    where $S$ denotes the tasks completed successfully.
    Notably, when combining tasks, a combined task counts as one task.
    \item \textbf{Average Completion Time (minutes, CT)}: The average time taken for completing tasks successfully.
        \begin{equation*}
            CT = \frac{\sum_{i \in S} T_i}{S}
        \end{equation*}
\end{itemize}

\kyle{vey cool metrics, I like this. }





\subsection{Main Results}

Based on the performance of language agents in Table~\ref{tab:main}, GPT-4 achieves the best performance across different task combinations. 
However, there is still room for improvement in cooking and laboratory scenarios\kyle{where can you see this result about cooking and laboratory? I'm confused}.
Moreover, the combined tasks are more challenging than single tasks despite the longer time given.
Apart from GPT-4, most models fail to complete 2 or 3 tasks, showing their limited multitasking abilities and the challenging nature of our environment.

For open-source models, OpenChat-3.5 and Vicuna-13B are even better than GPT-3.5, demonstrating their potential to develop multitasking capabilities.
However, although OpenChat-3.5 and Vicuna-13B exhibit faster completion speed and shorter average completion time than GPT-4, a lower task completion rate indicates that these models quickly complete simple actions initially but then encounter difficulties;
they either get caught in repetitive actions or fail to properly segment subsequent tasks, which significantly impacts task performance.
For example, initially, \coloredtexttt{potato} is unpicked, so the agent first performs \coloredtexttt{pick potato}. 
Subsequently, the agent mistakenly opts for \coloredtexttt{cook potato in pot} rather than the correct \coloredtexttt{chop potato},  due to its incorrectly decompose the task\kyle{grammar issue, fix, doesn't make sense}.














\subsection{Analysis}


\begin{figure}[t]
    \centering    
    \includegraphics[width=\linewidth]{figure/error.pdf}
    \caption{The proportions of correct and incorrect actions of each language agent.
    }
    \label{fig:error}
\end{figure}



\paragraph{Can language agents master multitasking?}
To further explore whether language agents can master multitasking, we conduct detailed analyses to investigate the types of actions these models can perform.
Based on environmental feedback, the actions are classified into two categories: correct ones and incorrect ones.
We further define 6 fine-grained types of actions, 
\ie, 
\textit{i)} correct actions: \textit{valid action}, \textit{wait}
\textit{ii)} incorrect actions: \textit{Invalid Action/Object)}, \textit{Dependency Violation}, \textit{Repeating Completed Action} and \textit{Object-Mismacthed Action}.\footnote{Detailed description of different types of actions can be found in Appendix~\ref{app:actiontype}.}
We calculate the frequency of these actions of each agent.\kyle{Maybe for later: this visualization makes it hard to see these correct/incorrect distinctions, should organization somehow the legend better, hard to interpret}

The results in Figure~\ref{fig:error} show that a significant proportion of invalid actions are due to dependency violations and mismatches with objects.
Multitasking involves performing several tasks simultaneously. 
As the number of tasks increases, the complexity of objects and actions escalates, leading to intricate dependencies between actions.
Thus, the high proportion of actions that violate dependencies and mismatch objects suggests that language agents face challenges in managing complex action interdependencies during multitasking, indicating a limitation in their multitasking capabilities.

\paragraph{Are language agents aware of parallel processing?}
Parallel processing can significantly reduce the time required for efficient multitasking. 
As stated in $\mathsection$~\ref{sec3:components}, we consider the duration of time for each action in \method to explore the parallel processing capabilities of language agents.
If an agent is capable of parallel processing,  it can engage in additional actions instead of waiting for the current action to complete.
However, as shown in Figure~\ref{fig:error}, we report the proportion of waiting actions across various models. 
The results reveal that waiting actions constitute over half of the valid actions performed by different LLMs.
This indicates a tendency for agents to engage in unnecessary waiting, which ignores parallel processing and leads to discrepancies in completion times as compared to the optimal in Table~\ref{tab:main}.\kyle{NOTE AGAIN: you didn't define precisely the optimal case and how it was computed. }

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/constraint.pdf}
    \caption{Comparison of the performance of GPT-4 with and without resource constraints. 
    We imposed constraints by limiting to a single instance each of \coloredtexttt{pot}, \coloredtexttt{fryer}, and \coloredtexttt{oven}.
    }
    \label{fig:constraint}
\end{figure}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figure/reward_curve.pdf}
    \caption{
    Task progress score curves of language agents on two task combinations in \method. %Each subfigure displays the progress score obtained by the agent over time.
    The names at the botton-right indicate the scenario and task number. 
    For example, \textit{cooking1} represents the first combination of tasks in the cooking scenario.
    }
    \label{fig:progress}
\end{figure*}

\paragraph{Do resource constraints affect the multitasking of language agents?}
Resource constraints refer to limitations in the availability of resources (\eg, the number of objects) necessary for task completion, which is rather common in real life.
To design resource constraints, we first select three objects: \coloredtexttt{pot}, \coloredtexttt{fryer} and \coloredtexttt{oven} in the cooking scenario, and adopt choose \# Task=2 setting in Table~\ref{tab:main}.
Then, we set that there is only one instance of each of the three objects, simulating the limitation of resources in the environment.
Figure~\ref{fig:constraint} compares GPT-4's performance before and after applying these constraints. 
We find that the constraints do not affect the task completion time or velocity, revealing that GPT-4 rarely attempts to process tasks in parallel.
However, a noticeable decline in both completion rate and progress score indicates that the constraints prevent the models from better comprehending and decomposing multiple tasks.








\paragraph{language agents misunderstand the state of the environment over time.}
To delve into the reason language agents struggle with multiple tasks, we analyze the progress score changes over time for various models.
As illustrated in Figure~\ref{fig:progress}, Vicuna, Mistral, and GPT-3.5 often cease scoring without completing all tasks, maintaining low scores until time runs out (\eg, (5,b), (2,c) and (6,d)).
We further examine their actions during these periods and find that they always perform \textbf{incorrect actions and waiting} alternately.
Since \coloredtexttt{wait} is a valid action, repeatedly alternating between waiting and incorrect actions does not lead to task failure, but neither does it contribute to an increase in scores.

To explain the behavior of consistently performing \textbf{incorrect actions and waiting}, we ask these models to explain the reason for each action, and the results show that these models believe \coloredtexttt{wait} can change object states, enabling invalid actions to succeed.
For example, The agent \coloredtexttt{wait} during \coloredtexttt{fry beef} and \coloredtexttt{beef} becomes \coloredtexttt{fried} after several minutes.
This indicates their flawed understanding of dynamic state changes in the environment and often results in them being trapped in infinite loops, ignoring environmental feedback.


==> archived/cons_three.tex <==
\begin{table*}[ht]
\centering
\caption{Model Performance under Different Task Numbers.CR($\uparrow$) CT($\downarrow$) AR($\uparrow$) CV($\uparrow$), we report the performance in cooking scenario}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
& \multicolumn{4}{c|}{\textbf{Three Task}} & \multicolumn{4}{c|}{\textbf{Three Task(constraint)}} \\
\cline{2-9}
& \textbf{CR} & \textbf{CT} & \textbf{AR} & \textbf{CV} & \textbf{CR} & \textbf{CT} & \textbf{AR} & \textbf{CV} \\
\hline
\multicolumn{9}{|c|}{\textit{Open Source Models}} \\
\hline
Mistral-7B  & 0 & 0 & 36.9 & 1.48 & 0 & 0 & 37.8 & 0.99 \\
Openchat-3.5 & 0 & 0 & 40.4 & 1.09 & 0 & 0 & 35.2 & 0.93 \\
Vicuna-13B & 0 & 0 & 38.6 & 1.66 & 0 & 0 & 15.8 & 0.89 \\
Mixtral-7Bx8 & 0 & 0 & 35.9 & 1.97 & 0 & 0 & 37.6 & 1.20 \\
\hline
\multicolumn{9}{|c|}{\textit{Closed Source Models}} \\
\hline
GPT-3.5 & 0 & 0 & 22.9 & 1.06 & 0 & 0 & 34.7 & 0.97 \\
GPT-4 & 60.0 & 75.33 & 90.7 & 1.24 & 50.0 & 80.6 & 84.4 & 1.21 \\
\hline
\end{tabular}
}
\label{tab:cons_two}
\end{table*}

==> archived/cons_two.tex <==
\begin{table*}[ht]
\small
\centering
\caption{Model Performance under Different Task Numbers.CR($\uparrow$) CT($\downarrow$) AR($\uparrow$) CV($\uparrow$), we report the performance in cooking scenario}
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
& \multicolumn{4}{c|}{\textbf{Two Task}} & \multicolumn{4}{c|}{\textbf{Two Task(constraint)}} \\
\cline{2-9}
& \textbf{CR} & \textbf{CT} & \textbf{AR} & \textbf{CV} & \textbf{CR} & \textbf{CT} & \textbf{AR} & \textbf{CV} \\
\hline
\multicolumn{9}{|c|}{\textit{Open Source Models}} \\
\hline
Mistral-7B  & 0 & 0 & 36.9 & 1.48 & 10.0 & 59.0 & 52.2 & 1.69 \\
Openchat-3.5 & 10.0 & 70.0 & 52.3 & 1.63 & 0 & 0 & 41.5 & 1.67  \\
Vicuna-13B & 0 & 0 & 38.6 & 1.66 & 0 & 0 & 40.0 & 1.63 \\
Mixtral-7Bx8 & 0 & 0 & 35.9 & 1.97 & 0 & 0 & 45.1 & 1.86 \\
\hline
\multicolumn{9}{|c|}{\textit{Closed Source Models}} \\
\hline
GPT-3.5 & 0 & 0 & 48.3 & 1.80 & 0 & 0 & 55.60 & 1.66  \\
GPT-4 & \textbf{70.0} & 52.71 & 92.8 & 1.83 & \textbf{50.00} & \textbf{51.8} & \textbf{92.7} & \textbf{1.81}  \\
\hline
\end{tabular}
\label{tab:cons_two}
\end{table*}

==> archived/objects.tex <==
\lstset{
    backgroundcolor=\color[RGB]{250,250,250},
    breaklines=true,
    breakindent=0pt,
    basicstyle=\ttfamily\small,
    frame=trbl,
    frameround = tttt,
}
\begin{table*}[!ht]
\toprule
"pick": "Pick the unpicked item.",
"cook in": "Cook the raw item until it's cooked through.",
"chop": "Chop the whole item into sliced pieces.",
"fry in": "Fry the raw item until it is fried to perfection.",
"wash": "Wash the dirty item to make clean.",
"bake in": "Bake the raw item in the oven until it's roasted.",
"activate": "Activate the inactive device to turn it active.",
"pour into": "Pour the liquid in item into the empty container until it is full.",
"brew with": "Brew the dry item leaves with the container until they're steeped.",
"gather": "Gather the scattered items until it is collected.",
"scrape into": "Scrape the contents from the full item into th empty item.",
"place into": "Place the unplaced item into the right place.",
"fill with": "Fill the container with something.",
"hoe": "Hoe the uncultivated item until it is cultivated and ready for planting.",
"weed_with": "Weed with the item.",
"set_up": "Set up the item that is not set yet until it is already set.",
"iron": "Iron the wrinkled item until they are smooth.",
"put on": "Put the item on the right place.",
"add to": "Add one item to the container.",
"rinse": "Rinse the dry item.",
"find": "Find the missed item so that it is found and can be used.",
"heat": "Heat the cool item until it is hot.",
"dilute": "Dilute the concentrated item until it is diluted.",
"cut": "Cut the whole item into divided pieces.",
"dissolve in": "Dissolve the solid item in the liquid until it is dissolved.",
"polish": "Polish the rusty item until it is polished.",
"empty": "Empty the full item until it is empty.",
"hanging": "Hang the item",
"water by": "Water the item by something",
"trim": "Trim the overgrown item",
"plant":"Plant the uncultivated item until it is planted",
"store": "Store the unstored item",
"stir with":"Stir the separate liquid in item with something until it is homogeneous",
"soak in": "Soak the dry item in something until it is wet",
"mop": "Mop the dirty item until it is clean",
"read": "Read the unknown item",
"fold": "Fold the spread item until it is tidy",
"crush": "Crush the intact item until it is crushed",
"cool": "Cool the hot item until it is cool",
"dry": "Dry the item until it is dry",
"wipe": "Wipe the dirty item until it is clean",
"put in": "Put the item in something",
"label": "Give the ambiguous item a label",
"crystallize": "Crystallize the fluid item until it is crystallized",
"filter": "Filter the mixed item until it is refined",

\caption{An example of \# Task=2 scenario}
\end{table*}
